Program Analysis via Multiple Context Free Language Reachability

Context-free language (CFL) reachability is a standard approach in static analyses, where the analysis question is phrased as a language reachability problem on a graph $G$ wrt a CFL L. While CFLs lack the expressiveness needed for high precision, common formalisms for context-sensitive languages are such that the corresponding reachability problem is undecidable. Are there useful context-sensitive language-reachability models for static analysis? In this paper, we introduce Multiple Context-Free Language (MCFL) reachability as an expressive yet tractable model for static program analysis. MCFLs form an infinite hierarchy of mildly context sensitive languages parameterized by a dimension $d$ and a rank $r$. We show the utility of MCFL reachability by developing a family of MCFLs that approximate interleaved Dyck reachability, a common but undecidable static analysis problem. We show that MCFL reachability be computed in $O(n^{2d+1})$ time on a graph of $n$ nodes when $r=1$, and $O(n^{d(r+1)})$ time when $r>1$. Moreover, we show that when $r=1$, the membership problem has a lower bound of $n^{2d}$ based on the Strong Exponential Time Hypothesis, while reachability for $d=1$ has a lower bound of $n^{3}$ based on the combinatorial Boolean Matrix Multiplication Hypothesis. Thus, for $r=1$, our algorithm is optimal within a factor $n$ for all levels of the hierarchy based on $d$. We implement our MCFL reachability algorithm and evaluate it by underapproximating interleaved Dyck reachability for a standard taint analysis for Android. Used alongside existing overapproximate methods, MCFL reachability discovers all tainted information on 8 out of 11 benchmarks, and confirms $94.3\%$ of the reachable pairs reported by the overapproximation on the remaining 3. To our knowledge, this is the first report of high and provable coverage for this challenging benchmark set.

==> app_normal_form.tex <==
\section{Proofs of \cref{SEC:NORMAL_FORM}}\label{SEC:APP_NORMAL_FORM}

==> figures/tab_insertion_mcfl.tex <==
\begin{table}
\caption{In progress, table of recognized strings for insertion language for $\IDL$, not filled} 
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|}
        \midrule
        \diagbox[width=1.5cm, height=0.7cm]{ d }{|s|} & 2 & 4 & 6 & 8 & 10 & 12\\
         \midrule
        1 & 2 & 6 & 18 & 56 & 180 & 594\\
        2 & 2 & 10 & 68 & 534 & 4552 & 40922\\
        total & 2 & 10 & 70 & 588 & 5544 & 56628\\
    \end{tabular}
    \label{table}
\end{table}
